Time Series Continuous Modeling for Imputation and Forecasting with Implicit Neural Representations

We introduce a novel modeling approach for time series imputation and forecasting, tailored to address the challenges often encountered in real-world data, such as irregular samples, missing data, or unaligned measurements from multiple sensors. Our method relies on a continuous-time-dependent model of the series' evolution dynamics. It leverages adaptations of conditional, implicit neural representations for sequential data. A modulation mechanism, driven by a meta-learning algorithm, allows adaptation to unseen samples and extrapolation beyond observed time-windows for long-term predictions. The model provides a highly flexible and unified framework for imputation and forecasting tasks across a wide range of challenging scenarios. It achieves state-of-the-art performance on classical benchmarks and outperforms alternative time-continuous models.

==> Experiments/figures/figure_forecast_train_test.tex <==
\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.99\linewidth]{Figures/train_test/forecasting_train_test.pdf}
    \caption{Comparison generalization setting ARTEMIS and Patch TST}
    \label{fig:train_test_forecast}
\end{figure}

==> Experiments/figures/figure_imputation_test_new_period.tex <==
\begin{figure*}[!htb]
    \centering
    \includegraphics[width=0.99\linewidth]{Figures/Procedure/imputation_new_samples_set_up.pdf}
    \caption{Procedure for imputation on new period for new samples}
    \label{fig:imputation_procedure_test}
\end{figure*}

==> Experiments/figures/figure_train_test_setting_Electricity.tex <==
\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Electricity/Imputations/train_test/train_electricity.pdf}
        \caption{MAE imputation error on train set. \textit{Electricity}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Electricity/Imputations/train_test/test_electricity.pdf}
        \caption{MAE imputation error on test set. \textit{Electricity}}
    \end{subfigure}
    \caption{Train/test setting on Electricity dataset.}
\end{figure*}

==> Experiments/figures/figure_train_test_setting_solar.tex <==
\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Solar/Imputation/train_test/train_solar.pdf}
        \caption{MAE imputation error on train set. \textit{Solar}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Solar/Imputation/train_test/test_solar.pdf}
        \caption{MAE imputation error on test set. \textit{Solar}}
    \end{subfigure}
    \caption{Train/test setting on Solar dataset.}
\end{figure*}

==> Experiments/figures/figure_train_test_setting_traffic.tex <==
\begin{figure*}[!htb]
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Traffic/Imputation/Train_test/train_traffic.pdf}
        \caption{MAE imputation error on train set. \textit{Traffic}}
    \end{subfigure}%
    ~ 
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=0.99\textwidth]{Figures/Traffic/Imputation/Train_test/test_traffic.pdf}
        \caption{MAE imputation error on test set. \textit{Traffic}}
    \end{subfigure}
    \caption{Train/test setting on Traffic dataset.}
\end{figure*}

==> Experiments/tables/table_datasets_info.tex <==
\begin{table}[H]
\renewcommand*{\arraystretch}{1.0}
\setlength{\tabcolsep}{4pt}
\caption{Summary of datasets information}
\label{tab:datasets infos}
\begin{center}
\scalebox{0.80}{%
\begin{tabular}{ccc}
\toprule[1.5pt]
    Dataset Name & Number of samples & Number of time steps  \\
        \midrule
    Electricity &  321               & 26304  \\
    Traffic     &  862               & 17544  \\
    Solar       &  137               & 52560  \\
    SolarH      & 137                & 8760   \\
        
        \bottomrule[1.5pt]

\end{tabular}}
\end{center}
\end{table}


==> Experiments/tables/table_forecast_and_impute_reverse.tex <==
\begin{table}[htbp]
\setlength{\tabcolsep}{4pt}
\caption{MAE results for forecasting on new samples on new period with missing values in the look-back window. Best results are in bold.}
\label{tab:flexibility_reverse}
\begin{center}
\resizebox{\linewidth}{!}{%
\begin{tabular}{cccccccccccccc}
\toprule
  & Datasets & \multicolumn{6}{c}{Electricity} & \multicolumn{6}{c}{Traffic} \\
  \cmidrule(r){3-8} \cmidrule(r){9-14} 
  
  & H & \multicolumn{3}{c}{96} & \multicolumn{3}{c}{192} & \multicolumn{3}{c}{96} & \multicolumn{3}{c}{192} \\

  \cmidrule(r){3-5} \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14} 
  
  & $\tau$ & 0.5 & 0.2 & 0.1 & 0.5 & 0.2 & 0.1 & 0.5 & 0.2 & 0.1 & 0.5 & 0.2 & 0.1\\                              

        \midrule
\multirow{2}{*}{ARTEMIS}                       & Imputation error & \textbf{0.184} & \textbf{0.245} & \textbf{0.357} & \textbf{0.184} & \textbf{0.250} & \textbf{0.372} & \textbf{0.219} & \textbf{0.278} & \textbf{0.418} & \textbf{0.211} & \textbf{0.271} & \textbf{0.397} \\
                                               & Forecast error   & \textbf{0.247} & \textbf{0.275} & \textbf{0.362} & \textbf{0.240} & \textbf{0.289} & \textbf{0.388} & \textbf{0.224} & \textbf{0.252} & \textbf{0.382} & \textbf{0.216} & \textbf{0.242} & \textbf{0.360} \\

                                    
        \cmidrule(r){2-14}
        
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Linear interpo \\ + Patch-TST\end{tabular}} 

& Imputation error & 0.257 & 0.482 & 0.663 & 0.258 & 0.481 & 0.669 & 0.276 &                                                   0.532 & 0.738 & 0.276 & 0.532 & 0.734 \\

& Forecast error   & 0.279 & 0.451 & 0.634 & 0.280 & 0.450 & 0.650 & 0.255 & 0.483 & 0.721 & 0.245 & 0.480 & 0.787 \\
        
        \bottomrule
  
\end{tabular}}
\end{center}
\end{table}



==> Experiments/tables/table_forecast_and_impute_short.tex <==
\begin{table}[H]
\renewcommand*{\arraystretch}{1.2}
\setlength{\tabcolsep}{5pt}
\caption{MAE results for forecasting on new samples and new period with missing values in the look-back window. Best results are in bold.}
\label{tab:flexibility}
\begin{center}
\scalebox{0.70}{%
\begin{tabular}{ccccccc}
\toprule[1.5pt]
  &   &        & \multicolumn{2}{c}{TimeFlow} & \multicolumn{2}{c}{Linear interpo $+$ PatchTST} \\
  
  \cmidrule(r){4-5} \cmidrule(r){6-7}                                       
  
  & H & $\tau$ & Imputation error & Forecast error & Imputation error & Forecast error\\
  
        \midrule

        %& 1.  & 0.000 $\pm$ 0.000 & 0.222 $\pm$ 0.031 & 0.000 $\pm$ 0.000 & 0.203 $\pm$ 0.037\\
\multirow{6}{*}{Traffic} & \multirow{3}{*}{96} & 0.5 & \textbf{0.219 $\pm$ 0.017} & \textbf{0.224 $\pm$ 0.033} & 0.276 $\pm$ 0.012 & 0.255 $\pm$ 0.041 \\
                                    &          & 0.2 & \textbf{0.278 $\pm$ 0.017} & \textbf{0.252 $\pm$ 0.029} & 0.532 $\pm$ 0.017 & 0.483 $\pm$ 0.040 \\
                                          &    & 0.1 & \textbf{0.418 $\pm$ 0.019} & \textbf{0.382 $\pm$ 0.014} & 0.738 $\pm$ 0.023 & 0.721 $\pm$ 0.073 \\

                    \cmidrule(r){2-7}
                    
                                       %& 1. & 0.000 $\pm$ 0.000 & 0.215 $\pm$ 0.026 & 0.000 $\pm$ 0.000 & 0.199 $\pm$ 0.030 \\
              &  \multirow{3}{*}{192}   & 0.5 & \textbf{0.211 $\pm$ 0.014} & \textbf{0.216 $\pm$ 0.028} & 0.276 $\pm$ 0.011 & 0.245 $\pm$ 0.029 \\
                                  &     & 0.2 & \textbf{0.271 $\pm$ 0.017} & \textbf{0.242 $\pm$ 0.026} & 0.532 $\pm$ 0.020 & 0.480 $\pm$ 0.050 \\
                                  &     & 0.1 & \textbf{0.397 $\pm$ 0.025} & \textbf{0.360 $\pm$ 0.022} & 0.734 $\pm$ 0.022 & 0.787 $\pm$ 0.172 \\
        
        \bottomrule[1.5pt]
  

\end{tabular}}
\end{center}
\end{table}



==> Experiments/tables/table_forecast_impute_full.tex <==
\begin{table}[!t]
\renewcommand*{\arraystretch}{1.4}
\setlength{\tabcolsep}{5pt}
\caption{MAE results for forecasting on new samples and new period with missing values in the look-back window. Best results are in bold.}
\label{tab:flexibility_complete_appendix}
\begin{center}
\scalebox{0.75}{%
\begin{tabular}{ccccccc}
\toprule[1.5pt]
  &   &        & \multicolumn{2}{c}{TimeFlow} & \multicolumn{2}{c}{Linear interpo $+$ PatchTST} \\
  
  \cmidrule(r){4-5} \cmidrule(r){6-7}                                       
  
  & H & $\tau$ & Imputation error & Forecast error & Imputation error & Forecast error\\
  
        \midrule
         \multirow{8}{*}{Electricity} & \multirow{4}{*}{96} & 1.  & 0.000 $\pm$ 0.000  & 0.241 $\pm$ 0.023 & 0.000 $\pm$ 0.000 & \textbf{0.224 $\pm$ 0.020} \\
         &    & 0.5 & \textbf{0.184 $\pm$ 0.004} & \textbf{0.247 $\pm$ 0.024} &  0.257 $\pm$ 0.008 & 0.279 $\pm$ 0.026 \\
                                      &                      & 0.2 & \textbf{0.245 $\pm$ 0.007} & \textbf{0.275 $\pm$ 0.027} & 0.482 $\pm$ 0.019 & 0.451 $\pm$ 0.042 \\
                                      &                      & 0.1 & \textbf{0.357 $\pm$ 0.016} & \textbf{0.362 $\pm$ 0.029} & 0.663 $\pm$ 0.029  & 0.634 $\pm$ 0.053\\

                            \cmidrule(r){2-7}
                    
                                        & \multirow{4}{*}{192} & 1. & 0.000 $\pm$ 0.000 & 0.254 $\pm$ 0.024 & 0.000 $\pm$ 0.000 &  \textbf{0.238 $\pm$ 0.024}\\
                                       &  & 0.5 & \textbf{0.184 $\pm$ 0.005} & \textbf{0.240 $\pm$ 0.026} & 0.258 $\pm$ 0.006 & 0.280 $\pm$ 0.032\\
                                       &                      & 0.2 & \textbf{0.250 $\pm$ 0.009} & \textbf{0.289 $\pm$ 0.029} & 0.481 $\pm$ 0.021 & 0.450 $\pm$ 0.054 \\
                                       &                      & 0.1 & \textbf{0.372 $\pm$ 0.017} & \textbf{0.388 $\pm$ 0.030} & 0.669 $\pm$ 0.030 & 0.650 $\pm$ 0.060 \\

        
        \midrule

        \multirow{8}{*}{Traffic} & \multirow{4}{*}{96} & 1.  & 0.000 $\pm$ 0.000 & 0.222 $\pm$ 0.031 & 0.000 $\pm$ 0.000 & \textbf{0.203 $\pm$ 0.037}\\
         &  & 0.5 & \textbf{0.219 $\pm$ 0.017} & \textbf{0.224 $\pm$ 0.033} & 0.276 $\pm$ 0.012 & 0.255 $\pm$ 0.041 \\
                                    &          & 0.2 & \textbf{0.278 $\pm$ 0.017} & \textbf{0.252 $\pm$ 0.029} & 0.532 $\pm$ 0.017 & 0.483 $\pm$ 0.040 \\
                                          &    & 0.1 & \textbf{0.418 $\pm$ 0.019} & \textbf{0.382 $\pm$ 0.014} & 0.738 $\pm$ 0.023 & 0.721 $\pm$ 0.073 \\

                    \cmidrule(r){2-7}
                    
                                       & \multirow{4}{*}{192} & 1. & 0.000 $\pm$ 0.000 & 0.215 $\pm$ 0.026 & 0.000 $\pm$ 0.000 & \textbf{0.199 $\pm$ 0.030} \\
              &   & 0.5 & \textbf{0.211 $\pm$ 0.014} & \textbf{0.216 $\pm$ 0.028} & 0.276 $\pm$ 0.011 & 0.245 $\pm$ 0.029 \\
                                  &     & 0.2 & \textbf{0.271 $\pm$ 0.017} & \textbf{0.242 $\pm$ 0.026} & 0.532 $\pm$ 0.020 & 0.480 $\pm$ 0.050 \\
                                  &     & 0.1 & \textbf{0.397 $\pm$ 0.025} & \textbf{0.360 $\pm$ 0.022} & 0.734 $\pm$ 0.022 & 0.787 $\pm$ 0.172 \\
        
        \bottomrule[1.5pt]
  

\end{tabular}}
\end{center}
\end{table}



==> Experiments/tables/table_forecasting_new_samples.tex <==
\begin{table}[H]
\renewcommand*{\arraystretch}{1.2}
\setlength{\tabcolsep}{4pt}
\caption{MAE results over horizon for the forecasting task in the context of generalization to new time series.}
\label{tab:forecast_new_samples}
\begin{center}
\scalebox{0.65}{%
\begin{tabular}{cccccc}
\toprule[1.5pt]
  & H &  \multicolumn{2}{c}{Known time series} & \multicolumn{2}{c}{New time series}\\
  \cmidrule(r){3-4} \cmidrule(r){5-6}

  &  & TimeFlow MAE error & PatchTST MAE error & TimeFlow MAE error & PatchTST MAE error \\
  
        \midrule

        \multirow{4}{*}{Electricity} & 96 & 0.228 $\pm$ 0.023 &  0.211 $\pm$ 0.007 & 0.241 $\pm$ 0.023 & 0.224 $\pm$ 0.020\\

        & 192  & 0.244 $\pm$ 0.022 & 0.225 $\pm$ 0.014 & 0.254 $\pm$ 0.024 &   0.238 $\pm$ 0.024 \\

        & 336 & 0.269 $\pm$ 0.036 & 0.267 $\pm$ 0.019 & 0.277 $\pm$ 0.033 &  0.285 $\pm$0.005 \\

        & 720 & 0.331 $\pm$ 0.058 &  0.310 $\pm$ 0.026 & 0.333 $\pm$ 0.059 &  0.331 $\pm$ 0.045\\

        
        \midrule

        \multirow{4}{*}{Traffic} & 96 & 0.226 $\pm$ 0.035 & 0.208 $\pm$ 0.036 & 0.222 $\pm$ 0.031 & 0.203 $\pm$ 0.037\\

        & 192 & 0.217 $\pm$ 0.028 & 0.202 $\pm$ 0.029 & 0.215 $\pm$ 0.026 & 0.199 $\pm$ 0.030 \\

        & 336 & 0.242 $\pm$ 0.036 & 0.228$\pm$ 0.041 & 0.240 $\pm$ 0.031 & 0.224$\pm$ 0.036\\

        & 720 & 0.283 $\pm$ 0.053 & 0.275 $\pm$ 0.059 & 0.283 $\pm$ 0.049 & 0.272$\pm$ 0.055\\
        
        \midrule


        \multirow{4}{*}{SolarH} & 96 & 0.237 $\pm$ 0.077 & 0.256 $\pm$ 0.055 & 0.236 $\pm$ 0.081 & 0.256 $\pm$ 0.062\\

        & 192 & 0.238 $\pm$ 0.051 & 0.251 $\pm$ 0.069 &  0.239 $\pm$ 0.058 & 0.250 $\pm$ 0.050\\

        & 336 & 0.220 $\pm$ 0.027 & 0.255 $\pm$ 0.066 & 0.220 $\pm$ 0.034 & 0.255 $\pm$ 0.066\\

        & 720 & 0.240 $\pm$ 0.039 & 0.267 $\pm$ 0.062 & 0.240 $\pm$ 0.042 & 0.267$\pm$ 0.063\\

        \midrule
         TimeFlow improvement & & / &  -1.05 $\%$ & / &  -0.39 $\%$ \\
        \bottomrule[1.5pt]

\end{tabular}}
\end{center}
\end{table}







==> Experiments/tables/table_imputation_generalization_new_samples.tex <==
\begin{table}[H]
\renewcommand*{\arraystretch}{1.4}
\setlength{\tabcolsep}{4pt}
\caption{MAE imputation error results for imputation on new periods for new sample setting}
\label{tab:impu_train_test}
\begin{center}
\scalebox{0.80}{%
\begin{tabular}{ccccc}
\toprule[1.5pt]
  &        &  \multicolumn{2}{c}{Known samples}        & New samples  \\
  
  \cmidrule(r){3-4} \cmidrule(r){5-5}   
  
  & $\tau$ &  \begin{tabular}{@{}c@{}}MAE error on the missing\\ grid for an observed period \end{tabular} & \begin{tabular}{@{}c@{}}MAE error on the missing\\ grid for unseen periods \end{tabular} & \begin{tabular}{@{}c@{}}MAE error on the missing\\grid for unseen periods \end{tabular}\\
        \midrule
        \multirow{3}{*}{Electricity} & 0.10 & 0.328 & 0.333 & 0.340\\

        & 0.30 & 0.277 & 0.279 & 0.281\\

        & 0.50 & 0.261 & 0.263 & 0.264\\

        \midrule
        \multirow{3}{*}{Traffic}& 0.10 &  & &\\

        & 0.30 & & &\\

        & 0.50 & & &\\
        
        \midrule
        \multirow{3}{*}{Solar}& 0.10 &  \\

        & 0.30 & & &\\

        & 0.50 & & &\\
        

        \bottomrule[1.5pt]

\end{tabular}}
\end{center}
\end{table}


==> Experiments/tables/table_imputation_train_test.tex <==
\begin{table}[H]
\renewcommand*{\arraystretch}{1.4}
\setlength{\tabcolsep}{4pt}
\caption{ARTEMIS MAE results for the generalization setting on new samples. $\tau$ stands for the sampling rate.}
\label{tab:impu_train_test}
\begin{center}
\scalebox{0.8}{%
\begin{tabular}{cccccc}
\toprule[1.5pt]
  & $\tau$ &  Fit error train & Imputation error train & Fit error test & Imputation error test\\
\midrule

        & 0.05 & 0.028 $\pm$ 0.001 & 0.368 $\pm$ 0.016 & 0.205 $\pm$ 0.013 & 0.393 $\pm$ 0.024\\

        & 0.10 & 0.020 $\pm$ 0.001 & 0.290 $\pm$ 0.009 & 0.233 $\pm$  0.013 &  0.306 $\pm$ 0.017\\

        Electricity & 0.20 & 0.036 $\pm$ 0.006 & 0.270 $\pm$ 0.011 & 0.229 $\pm$ 0.016 & 0.283$ \pm$ 0.019\\

        & 0.30 & 0.064 $\pm$ 0.024 & 0.249 $\pm$ 0.008 & 0.221 $\pm$ 0.014 & 0.262 $\pm$ 0.017\\

        & 0.50 & 0.081 $\pm$ 0.019 & 0.220 $\pm$ 0.009 & 0.213 $\pm$ 0.012 & 0.240 $\pm$ 0.014\\
        
        \midrule
        
        & 0.05 & 0.011 $\pm$ 0.002  & 0.103 $\pm$ 0.016 & 0.086 $\pm$ 0.013  & 0.113 $\pm$ 0.016 \\

        & 0.10 & 0.014 $\pm$ 0.002  & 0.091 $\pm$ 0.016 & 0.087 $\pm$ 0.014  & 0.105 $\pm$ 0.016 \\

        Solar & 0.20 & 0.024 $\pm$ 0.008  & 0.077 $\pm$ 0.014 & 0.087 $\pm$ 0.013  & 0.098 $\pm$ 0.015 \\

        & 0.30 & 0.033 $\pm$ 0.01 & 0.07 $\pm$ 0.014 & 0.087 $\pm$ 0.014 & 0.094 $\pm$ 0.014\\

        & 0.50 & 0.04 $\pm$ 0.012  & 0.062 $\pm$ 0.014 & 0.087 $\pm$ 0.013 & 0.091 $\pm$ 0.013\\
        
        \midrule

        & 0.05 & 0.035 $\pm$ 0.002 & 0.287 $\pm$ 0.014 & 0.139 $\pm$ 0.006 & 0.281 $\pm$ 0.011 \\

        & 0.10 & 0.025 $\pm$ 0.001 & 0.205 $\pm$ 0.010 & 0.148 $\pm$ 0.005 & 0.217 $\pm$ 0.008\\

        Traffic & 0.20 & 0.029 $\pm$ 0.006 & 0.172 $\pm$ 0.007  &  0.148 $\pm$ 0.007 & 0.191 $\pm$ 0.007\\

        & 0.30 & 0.039 $\pm$ 0.005 & 0.160 $\pm$ 0.006 & 0.144 $\pm$ 0.009 & 0.180 $\pm$ 0.007\\

        & 0.50 &  0.059 $\pm$ 0.004  & 0.155 $\pm$ 0.006 & 0.146  $\pm$ 0.005 & 0.173 $\pm$ 0.006\\

        \bottomrule[1.5pt]

\end{tabular}}
\end{center}
\end{table}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

